Pre-trained Large Language Models Use Fourier Features to Compute Addition

Pre-trained large language models (LLMs) exhibit impressive mathematical reasoning capabilities, yet how they compute basic arithmetic, such as addition, remains unclear. This paper shows that pre-trained LLMs add numbers using Fourier features -- dimensions in the hidden state that represent numbers via a set of features sparse in the frequency domain. Within the model, MLP and attention layers use Fourier features in complementary ways: MLP layers primarily approximate the magnitude of the answer using low-frequency features, while attention layers primarily perform modular addition (e.g., computing whether the answer is even or odd) using high-frequency features. Pre-training is crucial for this mechanism: models trained from scratch to add numbers only exploit low-frequency features, leading to lower accuracy. Introducing pre-trained token embeddings to a randomly initialized model rescues its performance. Overall, our analysis demonstrates that appropriate pre-trained representations (e.g., Fourier features) can unlock the ability of Transformers to learn precise mechanisms for algorithmic tasks.

==> trash/behavior.tex <==

%\section{Causal Tracing of Factual Associations} 
% \Tianyi{IDEA: To understand how the models achieve the correct answer in this manner, we examine the output of each MLP and attention module at every layer during prediction in Fourier space. We discover that the final prediction combines magnitude approximation and modular addition (Section \ref{sec:fourier_analysis}). We then apply a high-pass/low-pass filter to validate our hypothesis on how LLMs handle addition in Fourier space.}
% \Tianyi{comparing with \cite{stolfo2023a} we show that  attn  not just retrieve info but also do the computation}


==> trash/comments_not_to_arxiv.tex <==
%pre-trained large language models (LLMs) exhibit remarkable capabilities in executing tasks beyond their direct training objectives, yet the mechanisms through which they compute basic arithmetic, such as addition, remain largely unexplored.
\iffalse
Pre-trained large language models (LLMs) exhibit impressive mathematical reasoning capabilities, yet how they compute basic arithmetic, such as addition, remains unclear. 
% This paper investigates how pre-trained LLMs solve simple addition problems, focusing on the use of Fourier features in their computations. 
In this work, we show that pre-trained LLMs add numbers using their \textbf{Fourier features}.\Robin{This sentence needs to be made a little bit more exciting. It's also not clear to the reader what fourier features are}
First, through behavioral analysis, we show that LLMs do not merely memorize answers but instead compute them on the fly, progressively refining their predictions layer by layer. 
% By employing Fourier analysis, we dissect the contributions of MLP and attention modules within the model, revealing that MLP modules primarily contribute to magnitude approximation, whereas attention modules facilitate modular addition. 
Next, employing Fourier analysis \Robin{It's Fourier analysis + ablation study to get this result right? I would explain the ablation a bit more, I think it's quite central}, we reveal that MLP layers primarily approximate the magnitude of the answer, and attention layers facilitate modular addition (such as computing whether the answer has even or odd parity). 
% Furthermore, we demonstrate that these Fourier features are not an artifact of fine-tuning but are embedded during the pre-training phase. This is evidenced by distinct frequency components in pre-trained token embeddings, absent in models trained from scratch.
Fourier features are learned via pre-training: distinct frequency components in pre-trained token embeddings are absent in models trained from scratch.
Finally, we show that training the model from scratch but with pre-trained token embeddings incorporating Fourier features significantly boosts optimization convergence and accuracy. %This improvement is evident when compared to training the model from scratch with random initialization.\vatsal{Last sentence can be removed?}\Tianyi{yes}
%Our findings suggest a structured approach through which pre-trained LLMs process mathematical tasks, offering insights into their general problem-solving frameworks and highlighting the importance of pre-training for LLMs.
\fi


\iffalse
\Tianyi{
logit lens for pre-trained embedding + model from scratch
\begin{enumerate}
    \item For common language modeling task, the model store all the memory about that subject in the early site MLP and do the prediction at the end \cite{zhu2023physics, mbab22}.
    \item Inspired by \cite{nanda2023progress}, we do the Fourier analysis on the token embedding and intermediate state of the LLMs. We find that pre-trained model have already learned to embed the numbers in Fourier space and can quickly learn and accurately solve the problem. However, the model trained from scratch on math tasks does not learn the Fourier feature so that the accuracy is low.
    \item For the model that train on modular addition \cite{nanda2023progress}, there is no low-frequency components in the Fourier Space. The difference in addition is that there is also outlier low-frequency components.
    \item  In addition, on the logits heat plot, we can see that the late site module is doing both approximate and classification. We hypothesize that the low-frequency component is  approximating the magnitude of the result and the high-frequency is doing classification, i.e., modualr addition. For example, the component with period = 2 is checking the parity of the result.
    \item To better validate our hypothesis, we do ablation study. We drop the low-frequency components when predict and find that the model approximate the wrong result. For example, the model predict 159 instead of 59. When we drop high-frequency components, the model predict 58 instead of 59.
    \item We do causal tracing and Fourier analysis on other math tasks and get similar observations.
    \item We need to discuss the difference between addition task and modular addition tasks (with large $p$)
\end{enumerate}}



\Tianyi{

example of using nametag:

\Robin{}
\Deqing{}
\begin{enumerate}
\item Paper List:
\begin{itemize}
    \item \href{https://arxiv.org/pdf/2308.09124.pdf}{How relation information from sentences is extracted by the Transformer?}
    \item \href{https://arxiv.org/pdf/2202.05262.pdf}{Single fact memory editing} \cite{mbab22}
    \item \href{https://arxiv.org/pdf/2210.07229.pdf}{Multi-fact memory editing}
    \item \href{https://arxiv.org/pdf/2309.12284.pdf}{Math dataset which shows Transformer is bad at math/logic}
    \item \href{https://arxiv.org/pdf/2311.07618.pdf}{Evaluating the mathematical understanding of the GPT-4}
    \item 
     Other mathematical tasks like learning addition have
been used to investigate whether models possess algorithmic reasoning capabilities \cite{sgh+19,hbk+21,lad+22}
\end{itemize}


\item DONE List:
\begin{itemize}
\item fine tune gpt2 xl on \url{https://huggingface.co/datasets/math_dataset/viewer/arithmetic__add_or_sub} and compare the diff
\item fine tune gpt2-xl on math, plot the training loss, the eval metric

    \item \textbf{Causal Tracing Across Checkpoints:} 
    Test the causal tracing for each checkpoint to observe how the model gradually acquires the correct causal trace.
\end{itemize}

\item  ONGOING List:
\begin{itemize}
\item validate the hypothesis: \begin{center}
    {\it  The early site MLP store the property of the first operand. The attention modules in the middle layers of the last token gather the information about the operands and the operation. The late site takes these gathered information and do the computation.}
\end{center}

\item Test the casaul tracing on Llama 7b, change the evaluation method by the prediction acc

\item Compare the prediction for math data and language data when drop different number of layers

\item Use the idea in \href{https://arxiv.org/pdf/2401.06102.pdf}{https://arxiv.org/pdf/2401.06102.pdf} Section 4.1 to test whether the late site takes these gathered information and do the computation.
Use identity funtion and connect to unembedding layer.
Use a LRE and take the representation and do the computation. After learning that LRE, do the same compuation on other operands. (we can learn a LRE do addition and one for subtraction)

\end{itemize}

\item TODO List:
\begin{enumerate}
    \item \textbf{Dominance of MLP in Late Site Analysis:}
    \begin{itemize}
        \item Investigate the dominance of MLP in the late site, particularly when the third operand is corrupted.
        \item Explore the effects of restoring the early site MLP for the operand on the recovery of results.
        \item Examine implications of restoring late site MLP for the last token in the prompt on result recovery.
        \item Hypothesize if the result is pre-calculated and stored in the MLP memory.
    \end{itemize}

    \item \textbf{Recovery Across Different Layers:}
    \begin{itemize}
        \item Understand why restoring MLPs in different layers aids in result restoration.
        \item Question if memory is distributed across multiple layers instead of a single layer.
        \item Reference experiments involving the restoration of intervals of layers.
    \end{itemize}

    \item \textbf{Proposing Structural Improvements:}
    \begin{itemize}
        \item Suggest potential structural improvements for transformer model architectures.
    \end{itemize}

    \item \textbf{New Dataset Creation:}
    \begin{itemize}
        \item Create a dataset in the '$3,2,\times$; $1,4,+$' format, similar to the 'subject, relation, object' format in referenced research.
    \end{itemize}

    \item \textbf{Importance of First Half Layers of MLP:}
    \begin{itemize}
        \item Investigate the significance of the first half of the MLP layers.
    \end{itemize}

    \item \textbf{Understanding Operand and Operation Processing:}
    \begin{itemize}
        \item Explore how the model differentiates between operations like 12 - 3 and 3 - 12.
    \end{itemize}

    \item \textbf{Effect of Corrupting Relation Tokens:}
    \begin{itemize}
        \item Examine the impact of corrupting relation tokens and their properties stored in early site MLP.
    \end{itemize}

    \item \textbf{Post-Mid Site Attention Function:}
    \begin{itemize}
        \item Determine the necessary function post-mid site attention to compute the result.
    \end{itemize}

    \item \textbf{Controlled Dataset Creation:}
    \begin{itemize}
        \item Plan for creating a customized dataset for more controlled experimentation.
    \end{itemize}

    \item \textbf{Utilizing GPT-2 XL Tokenizer for Dataset:}
    \begin{itemize}
        \item Use the largest number token in GPT-2 XL tokenizer for dataset creation.
        \item Ensure all dataset components are within the token limits.
    \end{itemize}

    \item \textbf{Analysis of Attention Matrix at Specific Layers:}
    \begin{itemize}
        \item Inspect the attention matrix at layer 30 for information retrieval from the operands and operator MLP.
    \end{itemize}

    \item \textbf{Ignoring Attention in Last 10 Layers:}
    \begin{itemize}
        \item Test the prediction accuracy when ignoring attention in the last 10 layers.
    \end{itemize}

    \item \textbf{Impact of Corrupting MLP or Attention:}
    \begin{itemize}
        \item Study the changes in predictions when corrupting each MLP or attention component.
    \end{itemize}

    \item \textbf{Analyzing Transformer Computing Process:}
    \begin{itemize}
        \item Analyze the transformer's computation process by observing the output after adding MLP/attn residuals to the representation.
    \end{itemize}
    \item can we regard the addition computation MLP as the key-query memory structure in the ROME paper? it take 3,12,+ and do key query like early site mlp (retrieve memory) so that we can add some rules to that MLP? (like update memory)
\end{enumerate}


\end{enumerate}

}

\Tianyi{storyline: 
\begin{enumerate}
    \item when we do 12+3, the Causal tracing shows that restoring the late site MLP will also restore the predict result
    \item we guess the computation is done in the late site MLP so that the result is stored in the late site MLP
\end{enumerate}}
\fi



%intro


\iffalse
\Tianyi{we do not need that first paragraph, people have been using LLMs for math reasoning and solving, it leads to our first question. motivation 1 interested in doing math 2. intereptablilty understand how these models work. task with some good structure help easily understand. many prior works focus on small model like one-layer. no works shows how the pre-trained language models. with these two motivations and dive into what we do (constrast with other works like modular additon..)
one paragraph show what we observe in section 3 and one show how important pre-training is 
}

\iffalse
The artificial intelligence field has seen significant progress with the advent of large language models (LLMs), particularly marked by the development of the Transformer architecture.  This innovation has dramatically altered the landscape of natural language processing, particularly in fields such as machine translation \citep{prato2019fully, gao2020multi} and text generation \citep{luo2022biogpt}. As a result, models like BERT~\cite{dclt18}, PaLM~\cite{cnd+22}, LLaMA 2\cite{touvron2023llama2}, ChatGPT~\citep{chatgpt}, and GPT-4~\citep{openai23} have come to dominate the NLP domain.
\fi

The challenge of mathematical reasoning within large language models (LLMs) extends the boundaries of current understanding and tests the limits of artificial intelligence. While LLMs like GPT exhibit remarkable skill in generating human-like text, their effectiveness largely relies on pattern recognition from vast datasets. This observation prompts a critical inquiry: 
\begin{center}
    \textit{Do these models comprehend the underlying principles of mathematics, or are they merely parroting patterns learned during training?}
\end{center}
% This inquiry is particularly salient in light of Ilya Sutskever's assertion that GPT models learn representations of the processes that produce texts, effectively capturing aspects of the real world \cite{yc23}.
If we consider mathematics as a reflection of fundamental truths and logical structures of our world, then enabling LLMs to solve mathematical problems is not just about teaching them to perform calculations; it's about teaching them to understand a fundamental language of the universe. When a model like GPT-4 proves a theorem, is it demonstrating an understanding akin to human reasoning, or is it efficiently retrieving and recombining pieces of information it has been fed? \cite{yc23} stated that GPT-4’s ability is to reproduce,
rephrase, and polish the mathematical proofs that it has seen before, and not in
grasping mathematical concepts.


Building upon these insights, we aim to unravel how LLMs, specifically GPT models, handle basic arithmetic operations such as addition. Our primary question is: 
\begin{center}
\textit{How do pre-trained language models process and solve simple mathematical problems like $111+93=$?}
\end{center}
We first analyze the behavior of Large Language Models (LLMs) when performing arithmetic tasks in \S \ref{sec:behavioral_analysis}. We find that rather than merely retrieving answers from the training data, the models are capable of actually performing computations and progressively approaching the correct answer layer by layer. To understand how the models achieve the correct answer in this manner, we examine the output of each MLP and attention module at every layer during prediction in Fourier space. We discover that the final prediction combines magnitude approximation and modular addition (\S \ref{sec:fourier_analysis}). We then apply a high-pass/low-pass filter to validate our hypothesis on how LLMs handle addition in Fourier space. However, questions remain: Where do the models learn to utilize these Fourier features to solve addition problems, and why are these Fourier features necessary? To address these questions, in \S \ref{sec:effect_of_pre-training}, we demonstrate that LLMs can learn these Fourier features in the token embeddings for numbers during pre-training. We also illustrate how pre-training enhances the models' performance on addition tasks. In \S \ref{sec:express_addition}, we theoretically demonstrate how MLP and attention modules ca  represent modular addition and approximation to accurately compute the correct answers of addition. Finally, we validate our findings across other arithmetic tasks in \S \ref{sec:other_task}.
\Tianyi{we can say in section xx we show that the model is doing computation layer by layer}
% Our approach involves a series of causal tracing experiments and Fourier analysis. Following \cite{mbab22}, we first corrupt the elements of basic arithmetic expressions (e.g., the numbers and the plus sign) to analyze how the LLM stores memory about these individual components and how it processes them collectively (\S \ref{sec:causal_tracing}). We find that, comparing with other tasks, the late-site MLPs play important role to compute the correct answers. Next, we analyze the hidden states of the model during the prediction in Fourier space and find that the final prediction is the combination of magnitude approximation and modular addition (\S \ref{sec:fourier_analysis}). We then use the high-pass/low-pass filter to validate our hypothesis on how LLMs do addition in Fourier space (\S \ref{sec:filter}). Finally, we validate our statement in other arithmetic tasks (\S \ref{sec:other_task}).

\Tianyi{we need to emphasize that previous work only study on one-layer transformer modular addition task. We study on LLMs and addition task.}




\iffalse

In recent years, the capabilities of transformer language models like GPT in storing and recalling knowledge have piqued intense interest among AI researchers. Previous studies, such as \citep{mep20,mbab22}, have shed light on how these models retain factual associations within localized computations of middle-layer feed-forward modules. This revelation, further explored through techniques like the Rank-One Model Editing (ROME), has opened new pathways for directly modifying model weights to enhance factual recall.

The quest to endow LLMs with the capability to solve mathematical problems extends beyond a mere academic exercise; it touches the very core of what constitutes understanding in artificial intelligence. The conundrum arises from the fundamental nature of LLMs: while they demonstrate an astonishing ability to mimic human-like text generation, their proficiency largely stems from recognizing and replicating patterns in extensive textual data. This raises a pivotal question: do these models truly grasp the underlying logic of mathematics, or are they merely echoing patterns observed in their training datasets?

This inquiry is particularly salient in light of Ilya Sutskever's assertion that GPT models learn representations of the processes that produce texts, effectively capturing aspects of the real world \cite{yc23}. If we consider mathematics as a reflection of fundamental truths and logical structures of our world, then enabling LLMs to solve mathematical problems is not just about teaching them to perform calculations; it's about teaching them to understand a fundamental language of the universe. When a model like GPT-4 proves a theorem, is it demonstrating an understanding akin to human reasoning, or is it efficiently retrieving and recombining pieces of information it has been fed? \cite{yc23}  demonstrates that GPT-4 belongs to the latter one.

By delving into this challenge, we aim to discern whether LLMs can transcend the boundary of pattern recognition to engage in logical reasoning and genuine problem-solving. This endeavor holds the potential to redefine the boundaries of artificial intelligence, shifting from models that are proficient in text generation to ones that exhibit a deeper, more intrinsic understanding of complex concepts. It is a step towards a future where AI can not only mimic human thought processes but also independently engage with and solve problems that require a fundamental understanding of the world's logical and mathematical structure.


Building upon these insights, we propose to shift the focus from factual associations \cite{mbab22} to the realm of mathematical reasoning within LLMs. Mathematical operations, unlike factual recall, require a distinct kind of cognitive processing that involves both memory recall and logical computation. We aim to unravel how LLMs, specifically GPT models, handle basic arithmetic operations such as addition. Our primary question is: 
\begin{center}
\textit{How do LLMs process and solve simple mathematical problems like $2+3=$?}
\end{center}

Our approach involves a series of causal tracing experiments. Following \cite{mbab22}, we first corrupt the elements of basic arithmetic expressions (e.g., the numbers and the plus sign) to analyze how the LLM stores memory about these individual components and how it processes them collectively. We hypothesize that different parts of the equation might activate different areas of the LLMs, particularly the attention mechanisms, which could be pivotal in aggregating properties and performing calculations.

To better understand how transformer solve math problem, we train a smaller model specifically on mathematical operations to observe the solving process more closely. By comparing the neuron activations when solving different types of mathematical problems (e.g., '$3+12$' vs. '$3-10$'), we aim to understand the underlying mechanisms that guide LLMs in mathematical reasoning. 


Importantly, our study will also evaluate LLMs using a dataset by \cite{yc23} comprising mathematical problems and proofs not readily available online. Preliminary findings suggest that GPT-4's proficiency lies in reproducing and refining known mathematical proofs rather than understanding the underlying concepts. This approach will help identify GPT-4’s limitations in theorem proving and its reliance on previously encountered material.

A critical aspect of our study is to explore why LLMs exhibit limitations in logical reasoning and mathematical computation. By applying a structure analogous to the relation extraction in LRE \cite{hsh+23}, we intend to investigate if a different structure, capable of understanding logic, can be used to enhance the logical reasoning capabilities of LLMs.

\fi
\fi

% \Deqing{
% \begin{enumerate}
%     \item LLMs are bad at arithmetic/math. This motivates us to understand through interp how LLMs attempt to solve the problem.
%     \item First mention important prior works on interp. Prior interp work on math abilities focuses on one-layer model and trained from scratch. None of them work on pre-trained LMs. 
%     \item In this work, we investigate how \textit{pre-trained} LMs do addition.
%         \begin{enumerate}
%             \item they use Fourier features
%             \item MLP and Attn's roles
%             \item importance of pre-training
%         \end{enumerate}
% \end{enumerate}
% ------------------------Rewrite starts here----------------------------}


%\vspace{-2mm}
%\begin{center}
%    { \it Do these models \textit{comprehend} the underlying principles of mathematics, or do they merely \textit{parrot patterns} learned during training? }
%\end{center}
%\vspace{-2mm}

% Discuss related work, but first need to say what we do so the contrast is clear.
% This is really the "introduce the problem" paragraph, which includes saying how our problem differs from previously studied problems

\iffalse
such as greater-than \cite{hlv23}, greatest common divisor \cite{charton2023can}, linear regression \cite{Garg2022WhatCT,Oswald2022TransformersLI,Bai2023TransformersAS,fu2023transformers}, \Tianyi{We can just have one sentence for all other paper except the greater than}and modular addition \cite{nanda2023progress,gu2024fourier,Power2022GrokkingGB}. All of them 
% \Robin{Most or all? Be precise. Anything that studies the pre-trained model probably deserves more detailed discussion}\Tianyi{ It should be most. \cite{hlv23}  use the pre-trained GPT2 small model on greater than task. I changed the following sentence }
either study Transformers with a limited number of layers, or study Transformers trained from scratch, except for \cite{hlv23}, which uses the pre-trained GPT-2 small model on the greater than task. 
\fi

%By cutting short the residual stream at each MLP and attention module of each layer\Robin{ just say we use Logit Lens and cite}, we observe the final predictions combine magnitude approximation (in a multiple of 10, how large is $a + b$) and modular addition (what is $a + b \mod p$ for some number $p$). 
%Applying a high-pass or a low-pass filter to network modules,




%sec2

\iffalse
We constructed the ``language-math-dataset",\Robin{Can we come up with a better name for the dataset? You can make it a macro so it's easy to change} which consists of question-and-answer pairs that involve adding two numbers represented within a specific numerical system. Each pair is formulated to ensure that the resulting sum does not exceed $520$ \Robin{Say something about whether things are sampled uniformly at random}, the maximum number that can be represented by a single token in the GPT2-XL tokenizer. The dataset features questions sampled from five distinct formulations, such as ``What is the sum of $a$ and $b$?". For the sake of reproducibility and clarity, more detail is provided in the Appendix \ref{sec:detail_exp_setting}. \tzcomment{just say we construct a dataset ... without saying the name of the dataset}\tzcomment{We also create the ``format-math-dataset'' to show that our results generalize to other }\tzcomment{put the create dataset detail here}
\Robin{I think we should also talk about how much train/dev/test data there is in the main text}
\fi

%sec3

\iffalse
Each model layer use an attention module and a Multi-Layer Perceptron (MLP) module to perform additive updates to the token representation in the residual stream. At layer \(\ell\), for instance, where \(h^{(\ell)}\) is the current additive result of the token representation in the residual stream, the MLP and attention module update it as follows: 
\begin{align}\label{eq:residual_stream}
        h^{(\ell)}  = h^{(\ell-1)}  + \attn^{(\ell)}+ \mlp^{(\ell)}
\end{align}
with $ h^{(\ell)}  $ being the newly updated token representation  on the residual stream.  This process of updating $ h  $ with attention and MLP continues until the final model output, where the token representation is translated into vocabulary space through the language modeling head $W^{U} h^{(L)}$.
\fi

==> trash/exp.tex <==
\newpage
\section{Experiment}
\subsection{Pretrained GPT2-XL on Math Dataset}
Causal Traces \cite{mbab22} compute the causal effect of neuron activations by running the network on mathematical problems. Even though the GPT2-XL's prediction is wrong, we can see that the math operation activate the attention more and the number activate the MLP more. 

Additionally, the experiment results indicate that while the model primarily utilizes early-stage MLPs for initial computations and late-stage attention mechanisms for information synthesis, there is a degree of uncertainty in its data retrieval process. This can lead to inaccuracies in predictions due to occasional retrieval of information from incorrect locations within the model's architecture. Especially for the case that we corrupt the second number, the model fail to retrieve the property of them.
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answerstate.png}
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answermlp2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answerattn2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/What_is_3_plus_12_Answerstate2.png}
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answerstate.png}
    \caption{Indirect effect (IE) of 'Subtract 3 from 10. Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answermlp2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answerattn2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/pretrain/Subtract_3_from_10_Answerstate2.png}
    \caption{Indirect effect (IE) of 'Subtract 3 from 10. Answer:'}
    \label{fig:}
\end{figure}

\newpage
\subsection{Fine-tune GPT2-XL on Math Dataset}
We investigate the impact of fine-tuning on enhancing the mathematical computation capabilities of the Transformer model. By examining this aspect, insights into the Transformer's logical reasoning processes may be gleaned. The GPT2-XL model was selectively fine-tuned using a specialized mathematics dataset, focusing primarily on addition and subtraction operations\footnote{\url{https://huggingface.co/datasets/math_dataset/viewer/arithmetic__add_or_sub}}. Post fine-tuning, the model demonstrated a marked improvement in accurately computing results for identical inputs.
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answerstate.png}
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answermlp2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answerattn2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/What_is_3_plus_12_Answerstate2.png}
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answerstate.png}
    \caption{Indirect effect (IE) of 'Subtract 3 from 10. Answer:'}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answermlp2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answerattn2.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/Subtract_3_from_10_Answerstate2.png}
    \caption{Indirect effect (IE) of 'Subtract 3 from 10. Answer:'}
    \label{fig:}
\end{figure}

Compared with the pretrained version of GPT2-XL, the model manages to retrieve the information from a small range of MLP certainly.


As observed in \cite{mbab22}, there is the adaptation of the model's memory, particularly in the early layers of the Multi-Layer Perceptron (MLP). These layers appear to be fine-tuned for enhanced storage capabilities. Meanwhile, the later layers of the attention mechanism are responsible for aggregating information from previous tokens, culminating in the computation of the final result. 

However, our observations reveal a distinct pattern of causality, particularly notable in the 'late site' stages of the MLP during mathematical problem-solving tasks, a phenomenon not reported in \cite{mbab22}. For the last token in the prompt, the attention mechanism gains prominence in the intermediate stages, but the MLP also gains a dominant role in at late site.

% However, there are still some simple questions that finetuned GPT2-XL fail to answer.  There is also a degree of uncertainty in its data retrieval process, which lead to inaccuracies in predictions due to occasional retrieval of information from incorrect locations.


% This observed uncertainty might be attributed to the varied positions of token corruption. To explore this, the second number in the sequence was altered.
% \begin{figure}[!ht]
%     \vspace{-1em}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/3_+_5_Answer_mlp2.png}~
%     \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/3_+_5_Answer_attn2.png}~
%     \includegraphics[width=0.33\textwidth]{figures/gpt2xl/finetune/3_+_5_Answer_state2.png}
%     \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: '}
%     \label{fig:}
% \end{figure}

% The model correctly aggregates information from the appropriate location. However, the representation of '$5$' is notably less comprehensive compared to cases where the input is uncorrupted. This suggests that fine-tuning has not fully enabled the model to comprehend all aspects of the token '$5$'.
\newpage
\subsection{Fine-tune GPT2-XL on Formatted Math Dataset}
We change the format of the dataset to match the \{subject, relation, object\} format in \cite{mbab22} paper. For example, 'What is 3 plus 12? Answer: 15' is changed to '3  12  +  15'.

Before we finetune GPT2-XL on the new formatted data, the model predict the wrong results
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/'3'__12__+__mlp.png}~
   \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/'3'__12__+__attn.png}~ \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/'3'__12__+__state.png}~
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__'12'__+__mlp.png}~
   \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__'12'__+__attn.png}~
   \includegraphics[width=0.33\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__'12'__+__state.png}~
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__12__'+'__mlp.png}
   \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__12__'+'__attn.png} \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/pretrained/3__12__'+'__state.png}
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}
After finetuning, GPT2-XL manage to predict the results. We observe that MLP is also important in late site.
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/'3'__12__+__mlp.png}~
   \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/'3'__12__+__attn.png}~ \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/'3'__12__+__state.png}~
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}
\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__'12'__+__mlp.png}~
   \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__'12'__+__attn.png}~
   \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__'12'__+__state.png}~
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__12__'+'__mlp.png}
   \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__12__'+'__attn.png} \includegraphics[width=0.32\textwidth]{figures/gpt2xl-newdata/comparison/finetuned/3__12__'+'__state.png}
    \caption{Indirect effect (IE) of '3  12  + '}
    \label{fig:}
\end{figure}


We now have the new hypothesis:

\begin{center}
    {\it  The early site MLP store the property of the first operand. The attention modules in the middle layers of the last token gather the information about the operands and the operation. The late site takes these gathered information and do the computation.}
\end{center}
\subsection{How the Casual Tracing Changes when Fine-tuning}
\newpage
\subsubsection{Impact of Restoring MLP}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/24_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/66_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/114_What_is_3_plus_12_Answermlp.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 24, 66 and 114}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/126_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/180_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/210_What_is_3_plus_12_Answermlp.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 126, 180 and 210}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/252_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/2578_What_is_3_plus_12_Answermlp.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/16480_What_is_3_plus_12_Answermlp.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 252, 2578 and 16480}
    \label{fig:}
\end{figure}


\newpage
\subsubsection{Impact of Restoring Attention}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/24_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/66_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/114_What_is_3_plus_12_Answerattn.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 24, 66 and 114}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/126_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/180_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/210_What_is_3_plus_12_Answerattn.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 126, 180 and 210}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/252_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/2578_What_is_3_plus_12_Answerattn.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/16480_What_is_3_plus_12_Answerattn.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 252, 2578 and 16480}
    \label{fig:}
\end{figure}

\newpage
\subsubsection{Impact of Restoring State}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/24_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/66_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/114_What_is_3_plus_12_Answerstate.png}~
    \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 24, 66 and 114}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/126_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/180_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/210_What_is_3_plus_12_Answerstate.png}~
   \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 126, 180 and 210}
    \label{fig:}
\end{figure}

\begin{figure}[!ht]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/252_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/2578_What_is_3_plus_12_Answerstate.png}~
    \includegraphics[width=0.33\textwidth]{figures/gpt2xl/allcheckpoint/16480_What_is_3_plus_12_Answerstate.png}~
     \caption{Indirect effect (IE) of 'What is 3 plus 12? Answer: ' for checkpoints 252, 2578 and 16480}
    \label{fig:}
\end{figure}
